GCC: Generative Color Constancy via Diffusing a Color Checker

Color constancy methods often struggle to generalize across different camera sensors due to varying spectral sensitivities. We present GCC, which leverages diffusion models to inpaint color checkers into images for illumination estimation. Our key innovations include (1) a single-step deterministic inference approach that inpaints color checkers reflecting scene illumination, (2) a Laplacian decomposition technique that preserves checker structure while allowing illumination-dependent color adaptation, and (3) a mask-based data augmentation strategy for handling imprecise color checker annotations. By harnessing rich priors from pre-trained diffusion models, GCC demonstrates strong robustness in challenging cross-camera scenarios. These results highlight our method's effective generalization capability across different camera characteristics without requiring sensor-specific training, making it a versatile and practical solution for real-world applications.

==> figs/mask_da.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/mask_da.pdf}
    \caption{}
    \label{fig:mask_da}
\end{figure}

==> figs/pure_scene.tex <==
\begin{figure}[ht]
\vspace{-0.8pc}
    \centering
    \includegraphics[width=1\linewidth]{figures/pure_scene.pdf}
\vspace{-2pc}
    % \caption{TODO}
    % \label{fig:wo_pretrain}
\end{figure}

==> figs/wo_laplacian.tex <==
\begin{figure}[ht]
\vspace{-1pc}
    \centering
    \includegraphics[width=1\linewidth]{figures/wo_laplacian.pdf}
\vspace{-2pc}
    % \caption{TODO}
    % \label{fig:wo_pretrain}
\end{figure}

==> figs/wopretrain.tex <==
\begin{figure}[ht]
\vspace{-1pc}
    \centering
    \includegraphics[width=1\linewidth]{figures/wo_pretrain.pdf}
\vspace{-1pc}
    % \caption{TODO}
    % \label{fig:wo_pretrain}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

